BeyondEgo: Learning to Act Beyond Egocentric Perception via Humanoid Ego-Exo Foresight

Humanoid loco-manipulation requires coordinating whole-body motion to perform manipulation tasks in complex environments. Yet egocentric vision-language-action (VLA) policies can miss critical body--scene relationships, and action imitation alone provides no explicit supervision for future scene evolution. We propose BeyondEgo to extend VLA perception in space and time. Spatially, we encode a synchronized exocentric view with frozen DINOv3 and concatenate the resulting tokens with egocentric VLM tokens to condition the action expert. Temporally, we use future observations from both views as privileged supervision for a residual adapter on task-conditioned VLM features. A foresight expert regresses DINOv3 representations of both views 0.6s ahead. At deployment, the foresight expert is discarded and the 4.2M-parameter adapter is retained. We also introduce HELM, to our knowledge, the first closed-loop humanoid loco-manipulation benchmark with synchronized egocentric and exocentric views across five whole-body tasks. On HELM, BeyondEgo improves success from 48.0% to 92.0% in distribution and from 23.5% to 65.0% on 200 held-out scenes with layout, asset, material, and lighting shifts. Ablations show that dual-view DINOv3 foresight yields the best transfer results.

==> results.tex <==
\makeatletter
\newcommand{\BEm}[3]{\csname BE@m@#1@#2@#3\endcsname}
\newcommand{\BEa}[3]{\csname BE@a@#1@#2@#3\endcsname}
\newcommand{\BEs}[2]{\csname BE@s@#1@#2\endcsname}
\newcommand{\BEo}[2]{\csname BE@o@#1@#2\endcsname}
\newcommand{\BEf}[2]{\csname BE@f@#1@#2\endcsname}
\expandafter\def\csname BE@m@id@psi@1\endcsname{4}
\expandafter\def\csname BE@m@id@psi@1p\endcsname{4}
\expandafter\def\csname BE@m@id@s2@1\endcsname{8}
\expandafter\def\csname BE@m@id@s2@1p\endcsname{8}
\expandafter\def\csname BE@m@id@s1@1\endcsname{9}
\expandafter\def\csname BE@m@id@s1@1p\endcsname{9}
\expandafter\def\csname BE@m@id@full@1\endcsname{\textbf{10}}
\expandafter\def\csname BE@m@id@full@1p\endcsname{10}
\expandafter\def\csname BE@m@id@psi@2\endcsname{4}
\expandafter\def\csname BE@m@id@psi@2p\endcsname{4}
\expandafter\def\csname BE@m@id@s2@2\endcsname{9}
\expandafter\def\csname BE@m@id@s2@2p\endcsname{9}
\expandafter\def\csname BE@m@id@s1@2\endcsname{\textbf{10}}
\expandafter\def\csname BE@m@id@s1@2p\endcsname{10}
\expandafter\def\csname BE@m@id@full@2\endcsname{\textbf{10}}
\expandafter\def\csname BE@m@id@full@2p\endcsname{10}
\expandafter\def\csname BE@m@id@psi@3\endcsname{5}
\expandafter\def\csname BE@m@id@psi@3p\endcsname{5}
\expandafter\def\csname BE@m@id@s2@3\endcsname{7}
\expandafter\def\csname BE@m@id@s2@3p\endcsname{7}
\expandafter\def\csname BE@m@id@s1@3\endcsname{8}
\expandafter\def\csname BE@m@id@s1@3p\endcsname{8}
\expandafter\def\csname BE@m@id@full@3\endcsname{\textbf{9}}
\expandafter\def\csname BE@m@id@full@3p\endcsname{9}
\expandafter\def\csname BE@m@id@psi@4\endcsname{7}
\expandafter\def\csname BE@m@id@psi@4p\endcsname{7}
\expandafter\def\csname BE@m@id@s2@4\endcsname{7}
\expandafter\def\csname BE@m@id@s2@4p\endcsname{7}
\expandafter\def\csname BE@m@id@s1@4\endcsname{\textbf{9}}
\expandafter\def\csname BE@m@id@s1@4p\endcsname{9}
\expandafter\def\csname BE@m@id@full@4\endcsname{\textbf{9}}
\expandafter\def\csname BE@m@id@full@4p\endcsname{9}
\expandafter\def\csname BE@m@id@psi@5\endcsname{4}
\expandafter\def\csname BE@m@id@psi@5p\endcsname{4}
\expandafter\def\csname BE@m@id@s2@5\endcsname{6}
\expandafter\def\csname BE@m@id@s2@5p\endcsname{6}
\expandafter\def\csname BE@m@id@s1@5\endcsname{6}
\expandafter\def\csname BE@m@id@s1@5p\endcsname{6}
\expandafter\def\csname BE@m@id@full@5\endcsname{\textbf{8}}
\expandafter\def\csname BE@m@id@full@5p\endcsname{8}
\expandafter\def\csname BE@m@id@psi@sum\endcsname{24}
\expandafter\def\csname BE@m@id@psi@avg\endcsname{48.0}
\expandafter\def\csname BE@m@id@psi@avgb\endcsname{48.0}
\expandafter\def\csname BE@m@id@psi@ci\endcsname{[34.8, 61.5]}
\expandafter\def\csname BE@m@id@psi@n\endcsname{50}
\expandafter\def\csname BE@m@id@s2@sum\endcsname{37}
\expandafter\def\csname BE@m@id@s2@avg\endcsname{74.0}
\expandafter\def\csname BE@m@id@s2@avgb\endcsname{74.0}
\expandafter\def\csname BE@m@id@s2@ci\endcsname{[60.4, 84.1]}
\expandafter\def\csname BE@m@id@s2@n\endcsname{50}
\expandafter\def\csname BE@m@id@s1@sum\endcsname{42}
\expandafter\def\csname BE@m@id@s1@avg\endcsname{84.0}
\expandafter\def\csname BE@m@id@s1@avgb\endcsname{84.0}
\expandafter\def\csname BE@m@id@s1@ci\endcsname{[71.5, 91.7]}
\expandafter\def\csname BE@m@id@s1@n\endcsname{50}
\expandafter\def\csname BE@m@id@full@sum\endcsname{46}
\expandafter\def\csname BE@m@id@full@avg\endcsname{92.0}
\expandafter\def\csname BE@m@id@full@avgb\endcsname{\textbf{92.0}}
\expandafter\def\csname BE@m@id@full@ci\endcsname{[81.2, 96.8]}
\expandafter\def\csname BE@m@id@full@n\endcsname{50}
\expandafter\def\csname BE@m@gen@psi@1\endcsname{15}
\expandafter\def\csname BE@m@gen@psi@1p\endcsname{15}
\expandafter\def\csname BE@m@gen@s2@1\endcsname{25}
\expandafter\def\csname BE@m@gen@s2@1p\endcsname{25}
\expandafter\def\csname BE@m@gen@s1@1\endcsname{27}
\expandafter\def\csname BE@m@gen@s1@1p\endcsname{27}
\expandafter\def\csname BE@m@gen@full@1\endcsname{\textbf{31}}
\expandafter\def\csname BE@m@gen@full@1p\endcsname{31}
\expandafter\def\csname BE@m@gen@psi@2\endcsname{4}
\expandafter\def\csname BE@m@gen@psi@2p\endcsname{4}
\expandafter\def\csname BE@m@gen@s2@2\endcsname{20}
\expandafter\def\csname BE@m@gen@s2@2p\endcsname{20}
\expandafter\def\csname BE@m@gen@s1@2\endcsname{21}
\expandafter\def\csname BE@m@gen@s1@2p\endcsname{21}
\expandafter\def\csname BE@m@gen@full@2\endcsname{\textbf{25}}
\expandafter\def\csname BE@m@gen@full@2p\endcsname{25}
\expandafter\def\csname BE@m@gen@psi@3\endcsname{7}
\expandafter\def\csname BE@m@gen@psi@3p\endcsname{7}
\expandafter\def\csname BE@m@gen@s2@3\endcsname{17}
\expandafter\def\csname BE@m@gen@s2@3p\endcsname{17}
\expandafter\def\csname BE@m@gen@s1@3\endcsname{19}
\expandafter\def\csname BE@m@gen@s1@3p\endcsname{19}
\expandafter\def\csname BE@m@gen@full@3\endcsname{\textbf{24}}
\expandafter\def\csname BE@m@gen@full@3p\endcsname{24}
\expandafter\def\csname BE@m@gen@psi@4\endcsname{13}
\expandafter\def\csname BE@m@gen@psi@4p\endcsname{13}
\expandafter\def\csname BE@m@gen@s2@4\endcsname{30}
\expandafter\def\csname BE@m@gen@s2@4p\endcsname{30}
\expandafter\def\csname BE@m@gen@s1@4\endcsname{\textbf{35}}
\expandafter\def\csname BE@m@gen@s1@4p\endcsname{35}
\expandafter\def\csname BE@m@gen@full@4\endcsname{34}
\expandafter\def\csname BE@m@gen@full@4p\endcsname{34}
\expandafter\def\csname BE@m@gen@psi@5\endcsname{8}
\expandafter\def\csname BE@m@gen@psi@5p\endcsname{8}
\expandafter\def\csname BE@m@gen@s2@5\endcsname{7}
\expandafter\def\csname BE@m@gen@s2@5p\endcsname{7}
\expandafter\def\csname BE@m@gen@s1@5\endcsname{8}
\expandafter\def\csname BE@m@gen@s1@5p\endcsname{8}
\expandafter\def\csname BE@m@gen@full@5\endcsname{\textbf{16}}
\expandafter\def\csname BE@m@gen@full@5p\endcsname{16}
\expandafter\def\csname BE@m@gen@psi@sum\endcsname{47}
\expandafter\def\csname BE@m@gen@psi@avg\endcsname{23.5}
\expandafter\def\csname BE@m@gen@psi@avgb\endcsname{23.5}
\expandafter\def\csname BE@m@gen@psi@ci\endcsname{[18.2, 29.8]}
\expandafter\def\csname BE@m@gen@psi@n\endcsname{200}
\expandafter\def\csname BE@m@gen@s2@sum\endcsname{99}
\expandafter\def\csname BE@m@gen@s2@avg\endcsname{49.5}
\expandafter\def\csname BE@m@gen@s2@avgb\endcsname{49.5}
\expandafter\def\csname BE@m@gen@s2@ci\endcsname{[42.6, 56.4]}
\expandafter\def\csname BE@m@gen@s2@n\endcsname{200}
\expandafter\def\csname BE@m@gen@s1@sum\endcsname{110}
\expandafter\def\csname BE@m@gen@s1@avg\endcsname{55.0}
\expandafter\def\csname BE@m@gen@s1@avgb\endcsname{55.0}
\expandafter\def\csname BE@m@gen@s1@ci\endcsname{[48.1, 61.7]}
\expandafter\def\csname BE@m@gen@s1@n\endcsname{200}
\expandafter\def\csname BE@m@gen@full@sum\endcsname{130}
\expandafter\def\csname BE@m@gen@full@avg\endcsname{65.0}
\expandafter\def\csname BE@m@gen@full@avgb\endcsname{\textbf{65.0}}
\expandafter\def\csname BE@m@gen@full@ci\endcsname{[58.2, 71.3]}
\expandafter\def\csname BE@m@gen@full@n\endcsname{200}
\expandafter\def\csname BE@m@id@gain@full-psi\endcsname{44.0}
\expandafter\def\csname BE@m@id@gain@full-s1\endcsname{8.0}
\expandafter\def\csname BE@m@id@gain@s1-psi\endcsname{36.0}
\expandafter\def\csname BE@m@id@gain@s1-s2\endcsname{10.0}
\expandafter\def\csname BE@m@id@gain@s2-psi\endcsname{26.0}
\expandafter\def\csname BE@m@id@ratio@full-psi\endcsname{1.9}
\expandafter\def\csname BE@m@gen@gain@full-psi\endcsname{41.5}
\expandafter\def\csname BE@m@gen@gain@full-s1\endcsname{10.0}
\expandafter\def\csname BE@m@gen@gain@s1-psi\endcsname{31.5}
\expandafter\def\csname BE@m@gen@gain@s1-s2\endcsname{5.5}
\expandafter\def\csname BE@m@gen@gain@s2-psi\endcsname{26.0}
\expandafter\def\csname BE@m@gen@ratio@full-psi\endcsname{2.8}
\expandafter\def\csname BE@a@dinoego@id@1\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@1p\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@2\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@2p\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@3\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@3p\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@4\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@4p\endcsname{10}
\expandafter\def\csname BE@a@dinoego@id@pct\endcsname{100.0}
\expandafter\def\csname BE@a@dinoego@gen@1\endcsname{40}
\expandafter\def\csname BE@a@dinoego@gen@1p\endcsname{40}
\expandafter\def\csname BE@a@dinoego@gen@2\endcsname{35}
\expandafter\def\csname BE@a@dinoego@gen@2p\endcsname{35}
\expandafter\def\csname BE@a@dinoego@gen@3\endcsname{24}
\expandafter\def\csname BE@a@dinoego@gen@3p\endcsname{24}
\expandafter\def\csname BE@a@dinoego@gen@4\endcsname{24}
\expandafter\def\csname BE@a@dinoego@gen@4p\endcsname{24}
\expandafter\def\csname BE@a@dinoego@gen@pct\endcsname{60.0}
\expandafter\def\csname BE@a@dinoexo@id@1\endcsname{10}
\expandafter\def\csname BE@a@dinoexo@id@1p\endcsname{10}
\expandafter\def\csname BE@a@dinoexo@id@2\endcsname{10}
\expandafter\def\csname BE@a@dinoexo@id@2p\endcsname{10}
\expandafter\def\csname BE@a@dinoexo@id@3\endcsname{9}
\expandafter\def\csname BE@a@dinoexo@id@3p\endcsname{9}
\expandafter\def\csname BE@a@dinoexo@id@4\endcsname{9}
\expandafter\def\csname BE@a@dinoexo@id@4p\endcsname{9}
\expandafter\def\csname BE@a@dinoexo@id@pct\endcsname{90.0}
\expandafter\def\csname BE@a@dinoexo@gen@1\endcsname{40}
\expandafter\def\csname BE@a@dinoexo@gen@1p\endcsname{40}
\expandafter\def\csname BE@a@dinoexo@gen@2\endcsname{36}
\expandafter\def\csname BE@a@dinoexo@gen@2p\endcsname{36}
\expandafter\def\csname BE@a@dinoexo@gen@3\endcsname{27}
\expandafter\def\csname BE@a@dinoexo@gen@3p\endcsname{27}
\expandafter\def\csname BE@a@dinoexo@gen@4\endcsname{27}
\expandafter\def\csname BE@a@dinoexo@gen@4p\endcsname{27}
\expandafter\def\csname BE@a@dinoexo@gen@pct\endcsname{67.5}
\expandafter\def\csname BE@a@full@id@1\endcsname{10}
\expandafter\def\csname BE@a@full@id@1p\endcsname{10}
\expandafter\def\csname BE@a@full@id@2\endcsname{10}
\expandafter\def\csname BE@a@full@id@2p\endcsname{10}
\expandafter\def\csname BE@a@full@id@3\endcsname{9}
\expandafter\def\csname BE@a@full@id@3p\endcsname{9}
\expandafter\def\csname BE@a@full@id@4\endcsname{10}
\expandafter\def\csname BE@a@full@id@4p\endcsname{10}
\expandafter\def\csname BE@a@full@id@pct\endcsname{100.0}
\expandafter\def\csname BE@a@full@gen@1\endcsname{40}
\expandafter\def\csname BE@a@full@gen@1p\endcsname{40}
\expandafter\def\csname BE@a@full@gen@2\endcsname{39}
\expandafter\def\csname BE@a@full@gen@2p\endcsname{39}
\expandafter\def\csname BE@a@full@gen@3\endcsname{31}
\expandafter\def\csname BE@a@full@gen@3p\endcsname{31}
\expandafter\def\csname BE@a@full@gen@4\endcsname{\textbf{31}}
\expandafter\def\csname BE@a@full@gen@4p\endcsname{31}
\expandafter\def\csname BE@a@full@gen@pct\endcsname{77.5}
\expandafter\def\csname BE@a@qwenego@id@1\endcsname{10}
\expandafter\def\csname BE@a@qwenego@id@1p\endcsname{10}
\expandafter\def\csname BE@a@qwenego@id@2\endcsname{10}
\expandafter\def\csname BE@a@qwenego@id@2p\endcsname{10}
\expandafter\def\csname BE@a@qwenego@id@3\endcsname{8}
\expandafter\def\csname BE@a@qwenego@id@3p\endcsname{8}
\expandafter\def\csname BE@a@qwenego@id@4\endcsname{8}
\expandafter\def\csname BE@a@qwenego@id@4p\endcsname{8}
\expandafter\def\csname BE@a@qwenego@id@pct\endcsname{80.0}
\expandafter\def\csname BE@a@qwenego@gen@1\endcsname{40}
\expandafter\def\csname BE@a@qwenego@gen@1p\endcsname{40}
\expandafter\def\csname BE@a@qwenego@gen@2\endcsname{33}
\expandafter\def\csname BE@a@qwenego@gen@2p\endcsname{33}
\expandafter\def\csname BE@a@qwenego@gen@3\endcsname{17}
\expandafter\def\csname BE@a@qwenego@gen@3p\endcsname{17}
\expandafter\def\csname BE@a@qwenego@gen@4\endcsname{17}
\expandafter\def\csname BE@a@qwenego@gen@4p\endcsname{17}
\expandafter\def\csname BE@a@qwenego@gen@pct\endcsname{42.5}
\expandafter\def\csname BE@a@qwenexo@id@1\endcsname{10}
\expandafter\def\csname BE@a@qwenexo@id@1p\endcsname{10}
\expandafter\def\csname BE@a@qwenexo@id@2\endcsname{10}
\expandafter\def\csname BE@a@qwenexo@id@2p\endcsname{10}
\expandafter\def\csname BE@a@qwenexo@id@3\endcsname{9}
\expandafter\def\csname BE@a@qwenexo@id@3p\endcsname{9}
\expandafter\def\csname BE@a@qwenexo@id@4\endcsname{9}
\expandafter\def\csname BE@a@qwenexo@id@4p\endcsname{9}
\expandafter\def\csname BE@a@qwenexo@id@pct\endcsname{90.0}
\expandafter\def\csname BE@a@qwenexo@gen@1\endcsname{40}
\expandafter\def\csname BE@a@qwenexo@gen@1p\endcsname{40}
\expandafter\def\csname BE@a@qwenexo@gen@2\endcsname{37}
\expandafter\def\csname BE@a@qwenexo@gen@2p\endcsname{37}
\expandafter\def\csname BE@a@qwenexo@gen@3\endcsname{22}
\expandafter\def\csname BE@a@qwenexo@gen@3p\endcsname{22}
\expandafter\def\csname BE@a@qwenexo@gen@4\endcsname{22}
\expandafter\def\csname BE@a@qwenexo@gen@4p\endcsname{22}
\expandafter\def\csname BE@a@qwenexo@gen@pct\endcsname{55.0}
\expandafter\def\csname BE@a@qwenboth@id@1\endcsname{10}
\expandafter\def\csname BE@a@qwenboth@id@1p\endcsname{10}
\expandafter\def\csname BE@a@qwenboth@id@2\endcsname{10}
\expandafter\def\csname BE@a@qwenboth@id@2p\endcsname{10}
\expandafter\def\csname BE@a@qwenboth@id@3\endcsname{9}
\expandafter\def\csname BE@a@qwenboth@id@3p\endcsname{9}
\expandafter\def\csname BE@a@qwenboth@id@4\endcsname{9}
\expandafter\def\csname BE@a@qwenboth@id@4p\endcsname{9}
\expandafter\def\csname BE@a@qwenboth@id@pct\endcsname{90.0}
\expandafter\def\csname BE@a@qwenboth@gen@1\endcsname{39}
\expandafter\def\csname BE@a@qwenboth@gen@1p\endcsname{39}
\expandafter\def\csname BE@a@qwenboth@gen@2\endcsname{34}
\expandafter\def\csname BE@a@qwenboth@gen@2p\endcsname{34}
\expandafter\def\csname BE@a@qwenboth@gen@3\endcsname{25}
\expandafter\def\csname BE@a@qwenboth@gen@3p\endcsname{25}
\expandafter\def\csname BE@a@qwenboth@gen@4\endcsname{25}
\expandafter\def\csname BE@a@qwenboth@gen@4p\endcsname{25}
\expandafter\def\csname BE@a@qwenboth@gen@pct\endcsname{62.5}
\expandafter\def\csname BE@a@s1@id@4\endcsname{9}
\expandafter\def\csname BE@a@s1@id@4p\endcsname{9}
\expandafter\def\csname BE@a@s1@id@pct\endcsname{90.0}
\expandafter\def\csname BE@a@s1@gen@4\endcsname{27}
\expandafter\def\csname BE@a@s1@gen@4p\endcsname{27}
\expandafter\def\csname BE@a@s1@gen@pct\endcsname{67.5}
\expandafter\def\csname BE@a@adapteronly@id@4\endcsname{--}
\expandafter\def\csname BE@a@adapteronly@id@4p\endcsname{--}
\expandafter\def\csname BE@a@adapteronly@id@pct\endcsname{--}
\expandafter\def\csname BE@a@adapteronly@gen@4\endcsname{--}
\expandafter\def\csname BE@a@adapteronly@gen@4p\endcsname{--}
\expandafter\def\csname BE@a@adapteronly@gen@pct\endcsname{--}
\expandafter\def\csname BE@a@motcap@id@4\endcsname{--}
\expandafter\def\csname BE@a@motcap@id@4p\endcsname{--}
\expandafter\def\csname BE@a@motcap@id@pct\endcsname{--}
\expandafter\def\csname BE@a@motcap@gen@4\endcsname{--}
\expandafter\def\csname BE@a@motcap@gen@4p\endcsname{--}
\expandafter\def\csname BE@a@motcap@gen@pct\endcsname{--}
\expandafter\def\csname BE@s@s1@layout\endcsname{--}
\expandafter\def\csname BE@s@s1@asset\endcsname{--}
\expandafter\def\csname BE@s@s1@material\endcsname{--}
\expandafter\def\csname BE@s@s1@lighting\endcsname{--}
\expandafter\def\csname BE@s@s1@combined\endcsname{--}
\expandafter\def\csname BE@s@s1@total\endcsname{--}
\expandafter\def\csname BE@s@dinoego@layout\endcsname{4}
\expandafter\def\csname BE@s@dinoego@asset\endcsname{3}
\expandafter\def\csname BE@s@dinoego@material\endcsname{8}
\expandafter\def\csname BE@s@dinoego@lighting\endcsname{7}
\expandafter\def\csname BE@s@dinoego@combined\endcsname{2}
\expandafter\def\csname BE@s@dinoego@total\endcsname{24}
\expandafter\def\csname BE@s@dinoexo@layout\endcsname{6}
\expandafter\def\csname BE@s@dinoexo@asset\endcsname{3}
\expandafter\def\csname BE@s@dinoexo@material\endcsname{8}
\expandafter\def\csname BE@s@dinoexo@lighting\endcsname{7}
\expandafter\def\csname BE@s@dinoexo@combined\endcsname{3}
\expandafter\def\csname BE@s@dinoexo@total\endcsname{27}
\expandafter\def\csname BE@s@full@layout\endcsname{--}
\expandafter\def\csname BE@s@full@asset\endcsname{--}
\expandafter\def\csname BE@s@full@material\endcsname{--}
\expandafter\def\csname BE@s@full@lighting\endcsname{--}
\expandafter\def\csname BE@s@full@combined\endcsname{--}
\expandafter\def\csname BE@s@full@total\endcsname{--}
\expandafter\def\csname BE@s@qwenego@layout\endcsname{1}
\expandafter\def\csname BE@s@qwenego@asset\endcsname{3}
\expandafter\def\csname BE@s@qwenego@material\endcsname{6}
\expandafter\def\csname BE@s@qwenego@lighting\endcsname{5}
\expandafter\def\csname BE@s@qwenego@combined\endcsname{2}
\expandafter\def\csname BE@s@qwenego@total\endcsname{17}
\expandafter\def\csname BE@s@qwenexo@layout\endcsname{3}
\expandafter\def\csname BE@s@qwenexo@asset\endcsname{5}
\expandafter\def\csname BE@s@qwenexo@material\endcsname{7}
\expandafter\def\csname BE@s@qwenexo@lighting\endcsname{5}
\expandafter\def\csname BE@s@qwenexo@combined\endcsname{2}
\expandafter\def\csname BE@s@qwenexo@total\endcsname{22}
\expandafter\def\csname BE@s@qwenboth@layout\endcsname{3}
\expandafter\def\csname BE@s@qwenboth@asset\endcsname{3}
\expandafter\def\csname BE@s@qwenboth@material\endcsname{8}
\expandafter\def\csname BE@s@qwenboth@lighting\endcsname{7}
\expandafter\def\csname BE@s@qwenboth@combined\endcsname{4}
\expandafter\def\csname BE@s@qwenboth@total\endcsname{25}
\expandafter\def\csname BE@o@full@lossaction\endcsname{0.1311}
\expandafter\def\csname BE@o@full@cosego\endcsname{.951}
\expandafter\def\csname BE@o@full@cosexo\endcsname{.977}
\expandafter\def\csname BE@o@full@l1hand\endcsname{1.57}
\expandafter\def\csname BE@o@full@l1arm\endcsname{6.27}
\expandafter\def\csname BE@o@full@l1vx\endcsname{8.49}
\expandafter\def\csname BE@o@full@l1vy\endcsname{2.07}
\expandafter\def\csname BE@o@full@l1vyaw\endcsname{9.26}
\expandafter\def\csname BE@o@dinoego@lossaction\endcsname{0.1293}
\expandafter\def\csname BE@o@dinoego@cosego\endcsname{.951}
\expandafter\def\csname BE@o@dinoego@cosexo\endcsname{--}
\expandafter\def\csname BE@o@dinoego@l1hand\endcsname{1.63}
\expandafter\def\csname BE@o@dinoego@l1arm\endcsname{6.32}
\expandafter\def\csname BE@o@dinoego@l1vx\endcsname{8.89}
\expandafter\def\csname BE@o@dinoego@l1vy\endcsname{2.07}
\expandafter\def\csname BE@o@dinoego@l1vyaw\endcsname{8.08}
\expandafter\def\csname BE@o@dinoexo@lossaction\endcsname{0.1301}
\expandafter\def\csname BE@o@dinoexo@cosego\endcsname{--}
\expandafter\def\csname BE@o@dinoexo@cosexo\endcsname{.978}
\expandafter\def\csname BE@o@dinoexo@l1hand\endcsname{1.56}
\expandafter\def\csname BE@o@dinoexo@l1arm\endcsname{6.47}
\expandafter\def\csname BE@o@dinoexo@l1vx\endcsname{8.63}
\expandafter\def\csname BE@o@dinoexo@l1vy\endcsname{2.08}
\expandafter\def\csname BE@o@dinoexo@l1vyaw\endcsname{8.21}
\expandafter\def\csname BE@o@qwenego@lossaction\endcsname{0.1293}
\expandafter\def\csname BE@o@qwenego@cosego\endcsname{.946}
\expandafter\def\csname BE@o@qwenego@cosexo\endcsname{--}
\expandafter\def\csname BE@o@qwenego@l1hand\endcsname{1.63}
\expandafter\def\csname BE@o@qwenego@l1arm\endcsname{6.37}
\expandafter\def\csname BE@o@qwenego@l1vx\endcsname{8.75}
\expandafter\def\csname BE@o@qwenego@l1vy\endcsname{2.06}
\expandafter\def\csname BE@o@qwenego@l1vyaw\endcsname{7.82}
\expandafter\def\csname BE@o@qwenexo@lossaction\endcsname{0.1365}
\expandafter\def\csname BE@o@qwenexo@cosego\endcsname{--}
\expandafter\def\csname BE@o@qwenexo@cosexo\endcsname{.824}
\expandafter\def\csname BE@o@qwenexo@l1hand\endcsname{1.59}
\expandafter\def\csname BE@o@qwenexo@l1arm\endcsname{6.93}
\expandafter\def\csname BE@o@qwenexo@l1vx\endcsname{8.53}
\expandafter\def\csname BE@o@qwenexo@l1vy\endcsname{1.95}
\expandafter\def\csname BE@o@qwenexo@l1vyaw\endcsname{8.51}
\expandafter\def\csname BE@o@qwenboth@lossaction\endcsname{0.1314}
\expandafter\def\csname BE@o@qwenboth@cosego\endcsname{.946}
\expandafter\def\csname BE@o@qwenboth@cosexo\endcsname{.830}
\expandafter\def\csname BE@o@qwenboth@l1hand\endcsname{1.66}
\expandafter\def\csname BE@o@qwenboth@l1arm\endcsname{6.58}
\expandafter\def\csname BE@o@qwenboth@l1vx\endcsname{8.65}
\expandafter\def\csname BE@o@qwenboth@l1vy\endcsname{1.98}
\expandafter\def\csname BE@o@qwenboth@l1vyaw\endcsname{8.36}
\expandafter\def\csname BE@f@psi@l1hand\endcsname{1.26}
\expandafter\def\csname BE@f@psi@l1arm\endcsname{4.52}
\expandafter\def\csname BE@f@psi@l1vx\endcsname{11.68}
\expandafter\def\csname BE@f@psi@l1vy\endcsname{13.78}
\expandafter\def\csname BE@f@psi@l1vyaw\endcsname{21.48}
\expandafter\def\csname BE@f@s1@l1hand\endcsname{1.28}
\expandafter\def\csname BE@f@s1@l1arm\endcsname{5.20}
\expandafter\def\csname BE@f@s1@l1vx\endcsname{11.18}
\expandafter\def\csname BE@f@s1@l1vy\endcsname{11.74}
\expandafter\def\csname BE@f@s1@l1vyaw\endcsname{7.80}
\expandafter\def\csname BE@f@full@l1hand\endcsname{1.28}
\expandafter\def\csname BE@f@full@l1arm\endcsname{5.36}
\expandafter\def\csname BE@f@full@l1vx\endcsname{10.44}
\expandafter\def\csname BE@f@full@l1vy\endcsname{12.08}
\expandafter\def\csname BE@f@full@l1vyaw\endcsname{7.70}
\expandafter\def\csname BE@f@cosego@1\endcsname{0.950}
\expandafter\def\csname BE@f@cosego@2\endcsname{0.971}
\expandafter\def\csname BE@f@cosego@3\endcsname{0.955}
\expandafter\def\csname BE@f@cosego@4\endcsname{0.970}
\expandafter\def\csname BE@f@cosego@5\endcsname{0.967}
\expandafter\def\csname BE@f@cosego@mean\endcsname{0.963}
\expandafter\def\csname BE@f@cosexo@1\endcsname{0.975}
\expandafter\def\csname BE@f@cosexo@2\endcsname{0.981}
\expandafter\def\csname BE@f@cosexo@3\endcsname{0.990}
\expandafter\def\csname BE@f@cosexo@4\endcsname{0.986}
\expandafter\def\csname BE@f@cosexo@5\endcsname{0.986}
\expandafter\def\csname BE@f@cosexo@mean\endcsname{0.984}
\expandafter\def\csname BE@f@frames@1\endcsname{122{,}512}
\expandafter\def\csname BE@f@frames@2\endcsname{95{,}128}
\expandafter\def\csname BE@f@frames@3\endcsname{137{,}133}
\expandafter\def\csname BE@f@frames@4\endcsname{118{,}483}
\expandafter\def\csname BE@f@frames@5\endcsname{170{,}548}
\expandafter\def\csname BE@f@frames@total\endcsname{643{,}804}
\makeatother

